Phonon magnetochiral effect of band-geometric origin in Weyl semimetals

The phonon magnetochiral effect consists of a nonreciprocity in the velocity or attenuation of acoustic waves when they propagate parallel and antiparallel to an external magnetic field. The first experimental observation of this effect has been reported recently in a chiral magnet and ascribed to the hybridization between acoustic phonons and chiral magnons. Here, we predict a potentially measurable phonon magnetochiral effect of electronic origin in chiral Weyl semimetals. Caused by the Berry curvature and the orbital magnetic moment, this effect is enhanced for longitudinal phonons by the chiral anomaly.

==> refs1.tex <==
\begin{thebibliography}{100}
\makeatletter
\providecommand \@ifxundefined [1]{%
 \@ifx{#1\undefined}
}%
\providecommand \@ifnum [1]{%
 \ifnum #1\expandafter \@firstoftwo
 \else \expandafter \@secondoftwo
 \fi
}%
\providecommand \@ifx [1]{%
 \ifx #1\expandafter \@firstoftwo
 \else \expandafter \@secondoftwo
 \fi
}%
\providecommand \natexlab [1]{#1}%
\providecommand \enquote  [1]{``#1''}%
\providecommand \bibnamefont  [1]{#1}%
\providecommand \bibfnamefont [1]{#1}%
\providecommand \citenamefont [1]{#1}%
\providecommand \href@noop [0]{\@secondoftwo}%
\providecommand \href [0]{\begingroup \@sanitize@url \@href}%
\providecommand \@href[1]{\@@startlink{#1}\@@href}%
\providecommand \@@href[1]{\endgroup#1\@@endlink}%
\providecommand \@sanitize@url [0]{\catcode `\\12\catcode `\$12\catcode
  `\&12\catcode `\#12\catcode `\^12\catcode `\_12\catcode `\%12\relax}%
\providecommand \@@startlink[1]{}%
\providecommand \@@endlink[0]{}%
\providecommand \url  [0]{\begingroup\@sanitize@url \@url }%
\providecommand \@url [1]{\endgroup\@href {#1}{\urlprefix }}%
\providecommand \urlprefix  [0]{URL }%
\providecommand \Eprint [0]{\href }%
\providecommand \doibase [0]{http://dx.doi.org/}%
\providecommand \selectlanguage [0]{\@gobble}%
\providecommand \bibinfo  [0]{\@secondoftwo}%
\providecommand \bibfield  [0]{\@secondoftwo}%
\providecommand \translation [1]{[#1]}%
\providecommand \BibitemOpen [0]{}%
\providecommand \bibitemStop [0]{}%
\providecommand \bibitemNoStop [0]{.\EOS\space}%
\providecommand \EOS [0]{\spacefactor3000\relax}%
\providecommand \BibitemShut  [1]{\csname bibitem#1\endcsname}%
\let\auto@bib@innerbib\@empty
%</preamble>



\bibitem{reviews} For reviews, see e.g. M.Z. Hasan and C. L. Kane, \rmp {\bf 82}, 3045 (2010); X.-L. Qi and S.-C. Zhang, \rmp {\bf 83}, 1057 (2011); S. R. Elliott and M. Franz, \rmp {\bf 87}, 137 (2015); N. P. Armitage, E. J. Mele and A. Vishwanath, \rmp {\bf 90}, 015001 (2018).   
\bibitem{reviews2} For reviews, see e.g. N. R. Cooper, J. Dalibard and I. B. Spielman, \rmp {\bf 91}, 015005 (2019); T. Ozawa, H. M. Price, A. Amo, N. Goldman, M. Hafezi, L. Lu, M. C. Rechtsman, D. Schuster, J. Simon, O. Zilberberg and I. Carusotto, \rmp {\bf 91}, 015006 (2019); Y. Liu, X. Chen and Y. Xu, Adv. Funct. Mater. 2019, 1904784 (2019); X. Mao and T. C. Lubensky, Annu. Rev. Condens. Matter Phys. {\bf 9}, 413 (2018).
\bibitem{saha2015} K. Saha, K. L\'egar\'e and I. Garate, \prl {\bf 115}, 176405 (2015).
\bibitem{shapourian2015} H. Shapourian, T. L. Hughes and S. Ryu, \prb {\bf 92}, 165131 (2015).
\bibitem{cortijo2015} A. Cortijo, Y. Ferreir\'os, K. Landsteiner and M. A. H. Vozmediano, \prl {\bf 115}, 177202 (2015).
\bibitem{andreev2016} B. Z. Spivak and A. V. Andreev, \prb {\bf 93}, 085107 (2016).
\bibitem{song2016} Z. Song, J. Zhao, Z. Fang and X. Dai, \prb {\bf 94}, 214306 (2016).
\bibitem{rinkel2017} P. Rinkel, P. L. S. Lopes and I. Garate, \prl {\bf 119}, 107401 (2017).
\bibitem{rinkel2019} P. Rinkel, P. L. S. Lopes and I. Garate, \prb {\bf 99}, 144301 (2019).
\bibitem{chernodub2019} M. Chernodub and M. A. H. Vozmediano, Phys. Rev. Research {\bf 1}, 032040 (2019).
\bibitem{sukhachov2019} P. O. Sukhachov and H. Rostami, arXiv:1911.04526 (2019). 
\bibitem{rajaji2019} V. Rajaji, R. Arora, S. Ch. Sarma, B. Joseph, S. C. Peter, U. V. Waghmare and C. Narayana, \prb {\bf 99}, 184109 (2019).
\bibitem{laliberte2019} F. Lalibert\'e, F. B\'elanger, N. L. Lair, J. G. Analytis, M.-E. Boulanger, M. Dion, L. Taillefer and J. A. Quilliam, arXiv:1909.04270 (2019).
\bibitem{tokura2018} Y. Tokura, N. Nagaosa, Nature Communications {\bf 9}, 3740 (2018). 
\bibitem{nomura2019} T. Nomura, X.-X. Zhang, S. Zherlitsyn, J. Wosnitza, Y. Tokura, N. Nagaosa and S. Seki, \prl {\bf 122}, 145901 (2019).
\bibitem{huang2016} S.-M. Huang {\em et al.}, Proceedings of the National Academy of Sciences {\bf 113}, 1180 (2016).
\bibitem{chang2017} G. Chang {\em et al.}, \prl {\bf 119}, 206401 (2017).
\bibitem{tang2017} P. Tang, Q. Zhou and S.-C. Zhang, \prl {\bf 119}, 206402 (2017).
\bibitem{chang2018} G. Chang {\em et al.}, Nat. Mater. {\bf 17}, 978 (2018).
\bibitem{gooth2019} J. Gooth {\em et al.}, Nature {\bf 575}, 315 (2019).
\bibitem{rao2019} Z. Rao {\em et al.}, Nature {\bf 567}, 496 (2019).
\bibitem{sanchez2019} D. S. Sanchez {\em et al.}, Nature {\bf 567}, 500 (2019).
\bibitem{schroter2019} N. B. M.  Schr\"oter {\em et al.}, Nature Physics {\bf 15}, 759 (2019).
\bibitem{schroter2019b} N. B. M.  Schr\"oter {\em et al.}, arXiv:1907.08723 (2019).
\bibitem{shi2019} W. Shi {\em et al.}, arXiv:1909.04037 (unpublished).
\bibitem{takane2019} D. Takane {\em et al.}, \prl {\bf 122}, 076402 (2019).
\bibitem{dejuan2017} F. de Juan, A. G. Grushin, T. Morimoto and J. E. Moore, Nat. Commun. {\bf 8}, 15995 (2017); F. Flicker {\em et al.}, \prb {\bf 98}, 155145 (2018).
\bibitem{rees2019}  D. Rees {\em et al.}, arXiv:1902.03230 (unpublished)
\bibitem{zhang2018} T. Zhang, Z. Song, A. Alexandradinata, H. Weng, C. Fang, L. Lu and Z. Fang, \prl {\bf 120}, 016401 (2018).
\bibitem{liu2016} C.-X. Liu, S.-C. Zhang and X.-L. Qi, Annual Review of Condensed Matter Physics {\bf 7}, 301 (2016).
\bibitem{falkovsky} L. A. Falkovsky and E. G. Mischenko, \prb {\bf 51}, 7239 (1995); L. A. Falkovsky, \prb {\bf 66}, 020302 (R) (2002).
\bibitem{kontorovich1984} For a review, see e.g. V. M. Kontorovich, Sov. Phys. Usp. {\bf 27}, 134 (1984).
\bibitem{xiao2010} For a review, see e.g. D. Xiao, M.C. Chang and Q. Niu, \rmp {\bf 82}, 1959 (2010).
\bibitem{knoll2020} The comparable role of the Berry curvature and the orbital magnetic moment in the electronic transport properties of Weyl semimetals has been recently emphasized; see e.g. A. Knoll, C. Timm and T. Meng, \prb {\bf 101}, 201402 (2020).
\bibitem{kontorovich1963} V. M. Kontorovich, Sov. Phys. JETP {\bf 18}, 1638 (1963).
\bibitem{kontorovich1971} V. M. Kontorovich, Sov. Phys. JETP {\bf 32}, 11146 (1971).
\bibitem{song2019} Z. Song and X. Dai, Phys. Rev. X {\bf 9}, 021053 (2019).
\bibitem{sm} See the Supplemental Material for details on the solution of the Boltzmann equation and the elasticity equations.
\bibitem{zhong2015} S. Zhong, J. E. Moore and I. Souza, \prl {\bf 116}, 077201 (2016).
\bibitem{scalar} Here, ``scalar'' means invariant under any symmetry operation that is applied simultaneously to ${\bf q}$, ${\bf B}$ and the electronic structure. For instance, under inversion, we have ${\bf q}\to -{\bf q}$, ${\bf B}\to {\bf B}$ and the chiralities of the Weyl nodes are inverted.
\bibitem{nielsen1981} H. B. Nielsen and M. Ninomiya, Phys. Lett. B105, 219 (1981).
\bibitem{anastassakis1972}  See e.g. E. Anastassakis, E. Burstein, A. A. Maradudin and R. Minnick, J. Phys. Chem. Solids {\bf 33}, 1091 (1972).
\bibitem{similarities} A similar mechanism is in action in Ref. [\onlinecite{andreev2016}], where the calculated sound attenuation is proportional to $1/\Gamma_E$ (albeit quadratic in $B$). In addition, if one assumes a diagonal deformation potential tensor in Ref. [\onlinecite{andreev2016}], then only longitudinal phonons lead to a chiral imbalance.
\bibitem{jeff} J. Quilliam (private communication).
\bibitem{parameswaran2014} S. A. Parameswaran, T. Grover, D. A. Abanin, D. A. Pesin and A. Vishwanath, Phys. Rev. X {\bf 4}, 031035 (2014).
\bibitem{zhang2015} C.-L. Zhang {\em et al.}, Nature Communications {\bf 7}, 10735 (2016).
\bibitem{mehdi2019} M. Mehdi Jadidi, M. Kargarian, M. Mittendorff, Y. Aytac, B. Shen, J. C. K\"onig-Otto, S. Winnerl, N. Ni, A. L. Gaeta, T. E. Murphy, H. D. Drew, arXiv:1905.02236 (2019).


  
  

\end{thebibliography}
